Gravity, holography and applications to condensed matter

Momentum relaxation is an ever-present and unavoidable ingredient of any realistic condensed matter system. In real-world materials the presence of a lattice, impurities or disorder forces momentum to dissipate and leads to relevant physical effects such as the finiteness of the DC transport properties, i.e. conductivities. The main purpose of this thesis is the introduction of momentum dissipation and its consequent effects into the framework of AdS/CMT, namely the applications of the gauge-gravity duality to condensed matter. A convenient and effective way of breaking the translational symmetry associated to such a conservation law is provided by massive gravity (MG) bulk theories. We consider generic massive gravity models embedded into asymptotically Anti de Sitter spacetime and we analyze them using holographic techniques. We study in detail their consistency and stability. We then focus our attention on the transport properties of the CFT duals. A big part of our work is devoted to the analysis of the electric conductivity in relation to possible universal bounds and the existence of holographic metal-insulator transitions. We moreover initiate the study of the viscoelastic response and we consider the possible violation of the well known KSS bound. We finally describe the effects of momentum relaxation on the well known holographic models for superconductivity.

==> Bibliography/bibliography.tex <==
\begin{thebibliography}{99}
%\chapter*{Bibliography}
%
\addcontentsline{toc}{chapter}{Bibliography}


 \label{chapter:bibliography}
%\cite{Pohl:2010zza}
\bibitem{Pohl:2010zza}
  R.~Pohl {\it et al.},
  %``The size of the proton,''
  Nature {\bf 466} (2010) 213.
  %%CITATION = NATUA,466,213;%%

%\cite{Antognini:1900ns}
\bibitem{Antognini:1900ns} 
  A.~Antognini, F.~Nez, K.~Schuhmann, F.~D.~Amaro, F.~Biraben, J.~M.~R.~Cardoso, D.~S.~Covita and A.~Dax {\it et al.},
  %``Proton Structure from the Measurement of $2S-2P$ Transition Frequencies of Muonic Hydrogen,''
  Science {\bf 339}, 417 (2013).
  %%CITATION = SCIEA,339,417;%%
 
%\cite{Mohr:2012tt}
\bibitem{Mohr:2012tt} 
  P.~J.~Mohr, B.~N.~Taylor and D.~B.~Newell,
  %``CODATA Recommended Values of the Fundamental Physical Constants: 2010,''
  Rev.\ Mod.\ Phys.\  {\bf 84}, 1527 (2012)
  [arXiv:1203.5425 [physics.atom-ph]].
  %%CITATION = ARXIV:1203.5425;%%
  
%\cite{Lorenz:2014vha}
\bibitem{Lorenz:2014vha} 
  I.~T.~Lorenz and U.-G.~Meiner,
  %``Reduction of the proton radius discrepancy by 3 sigma,''
  arXiv:1406.2962 [hep-ph].
  %%CITATION = ARXIV:1406.2962;%%

%\cite{Pineda:2002as}
\bibitem{Pineda:2002as}
  A.~Pineda,
  %``Leading chiral logs to the hyperfine splitting of the hydrogen and muonic
  %hydrogen,''
  Phys.\ Rev.\  C {\bf 67}, 025201 (2003)
  [arXiv:hep-ph/0210210];
  %%CITATION = PHRVA,C67,025201;%%
  %\cite{Pineda:2003hb}
  A.~Pineda,
  %``Learning about the chiral structure of the proton from the hyperfine splitting,''
  hep-ph/0308193.
  %%CITATION = HEP-PH/0308193;%%
 
%\cite{Pineda:2004mx}
\bibitem{Pineda:2004mx}
  A.~Pineda,
  %``The Chiral structure of the Lamb shift and the definition of the proton
  %radius,''
  Phys.\ Rev.\  C {\bf 71}, 065205 (2005)
  [arXiv:hep-ph/0412142].
  %%CITATION = PHRVA,C71,065205;%%
  
%\cite{Nevado:2007dd}
\bibitem{Nevado:2007dd}
  D.~Nevado and A.~Pineda,
  %``Forward virtual Compton scattering and the Lamb shift in chiral
  %perturbation theory,''
  Phys.\ Rev.\  C {\bf 77}, 035202 (2008)
  [arXiv:0712.1294 [hep-ph]].
  %%CITATION = PHRVA,C77,035202;%%

%\cite{Pineda:2011xp}
\bibitem{Pineda:2011xp} 
  A.~Pineda,
  %``Brief review of the theory of the muonic hydrogen Lamb shift and the proton radius,''
  arXiv:1108.1263 [hep-ph].
  %%CITATION = ARXIV:1108.1263;%%

%\cite{Jenkins:1990jv}
\bibitem{Jenkins:1990jv} 
  E.~E.~Jenkins and A.~V.~Manohar,
  %``Baryon chiral perturbation theory using a heavy fermion Lagrangian,''
  Phys.\ Lett.\ B {\bf 255}, 558 (1991).
  %%CITATION = PHLTA,B255,558;%%
 
%\cite{Bernard:1992qa}
\bibitem{Bernard:1992qa} 
  V.~Bernard, N.~Kaiser, J.~Kambor and U.~G.~Meissner,
  %``Chiral structure of the nucleon,''
  Nucl.\ Phys.\ B {\bf 388}, 315 (1992).
  %%CITATION = NUPHA,B388,315;%%

%\cite{Caswell:1985ui}
\bibitem{Caswell:1985ui} 
  W.~E.~Caswell and G.~P.~Lepage,
  %``Effective Lagrangians for Bound State Problems in QED, QCD, and Other Field Theories,''
  Phys.\ Lett.\ B {\bf 167}, 437 (1986).
  %%CITATION = PHLTA,B167,437;%%
 
%\cite{Pineda:1997bj}
\bibitem{Pineda:1997bj}
  A.~Pineda and J.~Soto,
  %``Effective field theory for ultrasoft momenta in NRQCD and NRQED,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 64}, 428 (1998)
  [arXiv:hep-ph/9707481].
  %%CITATION = NUPHZ,64,428;%%

%\cite{Pineda:1997ie}
\bibitem{Pineda:1997ie} 
  A.~Pineda and J.~Soto,
  %``The Lamb shift in dimensional regularization,''
  Phys.\ Lett.\ B {\bf 420}, 391 (1998)
  [hep-ph/9711292].
  %%CITATION = HEP-PH/9711292;%%
  
%\cite{Pineda:1998kn}
\bibitem{Pineda:1998kn}
  A.~Pineda and J.~Soto,
  %``Potential NRQED: The Positronium case,''
  Phys.\ Rev.\  D {\bf 59}, 016005 (1999)
  [arXiv:hep-ph/9805424].
  %%CITATION = PHRVA,D59,016005;%%

%\cite{Peset:2014jxa}
\bibitem{Peset:2014jxa} 
  C.~Peset and A.~Pineda,
  %``The two-photon exchange contribution to muonic hydrogen from chiral perturbation theory,''
  arXiv:1406.4524 [hep-ph].
  %%CITATION = ARXIV:1406.4524;%%

%\cite{Kinoshita:1998jf}
\bibitem{Kinoshita:1998jf} 
  T.~Kinoshita and M.~Nio,
  %``Sixth order vacuum polarization contribution to the Lamb shift of the muonic hydrogen,''
  Phys.\ Rev.\ Lett.\  {\bf 82}, 3240 (1999)
  [Erratum-ibid.\  {\bf 103}, 079901 (2009)]
  [hep-ph/9812442].
  %%CITATION = HEP-PH/9812442;%%
  
%\cite{Ivanov:2009aa}
\bibitem{Ivanov:2009aa} 
  V.~G.~Ivanov, E.~Y.~Korzinin and S.~G.~Karshenboim,
  %``Comment on `Sixth-Order Vacuum-Polarization Contribution to the Lamb Shift of Muonic Hydrogen' by T. Kinoshita and M. Nio, Phys.Rev. Lett.82,3240 (1999),''
  arXiv:0905.4471 [physics.atom-ph].
  %%CITATION = ARXIV:0905.4471;%%
  
%\cite{Karshenboim:2010cq}
\bibitem{Karshenboim:2010cq} 
  S.~G.~Karshenboim, E.~Y.~Korzinin, V.~G.~Ivanov and V.~A.~Shelyuto,
  %``Contribution of Light-by-Light Scattering to Energy Levels of Light Muonic Atoms,''
  JETP Lett.\  {\bf 92}, 8 (2010)
  [arXiv:1005.4880 [physics.atom-ph]].
  %%CITATION = ARXIV:1005.4880;%%
  
\bibitem{pachucki1} K. Pachucki, Phys. Rev. {\bf A53}, 2092 (1996).

 %\cite{Veitia}
\bibitem{Veitia}
  A.~Veitia and K.~Pachucki,
  %``Nuclear recoil effects in antiprotonic and muonic atoms,''
  Phys.\ Rev.\ A {\bf 69} (2004) 042501.
  %%CITATION = PHRVA,A69,042501;%%
 
 %\cite{Borie:2012zz}
\bibitem{Borie:2012zz} 
  E.~Borie,
  %``Lamb shift in light muonic atoms: Revisited,''
  Annals Phys.\  {\bf 327}, 733 (2012).
  %%CITATION = APNYA,327,733;%%
 
 %\cite{Jentschura:2011nx}
\bibitem{Jentschura:2011nx}
  U.~D.~Jentschura,
  %``Relativistic Reduced-Mass and Recoil Corrections to Vacuum Polarization in Muonic Hydrogen, Muonic Deuterium and Muonic Helium Ions,''
  Phys.\ Rev.\ A {\bf 84} (2011) 012505
  [arXiv:1107.1737 [physics.atom-ph]].
  %%CITATION = ARXIV:1107.1737;%%
 
\bibitem{KIK}
 S.~G.~Karshenboim,   V.~G.~Ivanov and E.~Y.~Korzinin,
  Phys.\ Rev.\ A {\bf 85} (2012) 032509.
 
 %\cite{Barbieri:1973kk}
\bibitem{Barbieri:1973kk}
 R.~Barbieri, M.~Caffo and E.~Remiddi,
  %``Fourth-order charge radius of the muon and its contribution to the lamb shift,''
  Lett.\ Nuovo Cim.\  {\bf 7S2} (1973) 60
   [Lett.\ Nuovo Cim.\  {\bf 7} (1973) 60].
  %%CITATION = NCLTA,7S2,60;%%
 
%\cite{Barbieri:1972as}
\bibitem{Barbieri:1972as}
  R.~Barbieri, J.~A.~Mignaco and E.~Remiddi,
  %``Electron form-factors up to fourth order. 1.,''
  Nuovo Cim.\ A {\bf 11} (1972) 824.
  %%CITATION = NUCIA,A11,824;%%
  
%\cite{Pineda:2002bv}
\bibitem{Pineda:2002bv} 
  A.~Pineda,
  %``Renormalization group improvement of the spectrum of hydrogen - like atoms with massless fermions,''
  Phys.\ Rev.\ A {\bf 66}, 062108 (2002)
  [hep-ph/0204213].
  %%CITATION = HEP-PH/0204213;%%
   
%\cite{Jentschura:2011ck}
\bibitem{Jentschura:2011ck} 
  U.~D.~Jentschura and B.~J.~Wundt,
  %``Semi-Analytic Approach to Higher-Order Corrections in Simple Muonic Bound Systems: Vacuum Polarization, Self-Energy and Radiative-Recoil,''
  Eur.\ Phys.\ J.\ D {\bf 65}, 357 (2011)
  [arXiv:1112.0556 [physics.atom-ph]].
  %%CITATION = ARXIV:1112.0556;%%
 
%\cite{Korzinin:2013uia}
\bibitem{Korzinin:2013uia} 
  E.~Y.~Korzinin, V.~G.~Ivanov and S.~G.~Karshenboim,
  %``The $\alpha^2(Z\alpha)^4m$ contributions to the Lamb shift and the fine structure in light muonic atoms,''
  arXiv:1311.5784 [physics.atom-ph].
  %%CITATION = ARXIV:1311.5784;%%
  
%\cite{Friar:1978wv}
\bibitem{Friar:1978wv} 
  J.~L.~Friar,
  %``Nuclear Finite Size Effects in Light Muonic Atoms,''
  Annals Phys.\  {\bf 122}, 151 (1979).
  %%CITATION = APNYA,122,151;%%
  
%\cite{Jegerlehner:1996ab}
\bibitem{Jegerlehner:1996ab} 
  F.~Jegerlehner,
  %``Hadronic vacuum polarization contribution to g-2 of the leptons and alpha (M(Z)),''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 51C}, 131 (1996)
  [hep-ph/9606484].
  %%CITATION = HEP-PH/9606484;%%
 
%\cite{Jenkins:1991es}
\bibitem{Jenkins:1991es} 
  E.~E.~Jenkins and A.~V.~Manohar,
  %``Chiral corrections to the baryon axial currents,''
  Phys.\ Lett.\ B {\bf 259}, 353 (1991).
  %%CITATION = PHLTA,B259,353;%%

%\cite{Dashen:1993ac}
\bibitem{Dashen:1993ac} 
  R.~F.~Dashen and A.~V.~Manohar,
  %``1/N(c) corrections to the baryon axial currents in QCD,''
  Phys.\ Lett.\ B {\bf 315}, 438 (1993)
  [hep-ph/9307242].
  %%CITATION = HEP-PH/9307242;%%
  %190 citations counted in INSPIRE as of 05 Mar 2014

%\cite{Pachucki:1999zza}
\bibitem{Pachucki:1999zza} 
  K.~Pachucki,
  %``Proton structure effects in muonic hydrogen,''
  Phys.\ Rev.\ A {\bf 60}, 3593 (1999).
  %%CITATION = PHRVA,A60,3593;%%

%\cite{Carlson:2011zd}
\bibitem{Carlson:2011zd} 
  C.~E.~Carlson and M.~Vanderhaeghen,
  %``Higher order proton structure corrections to the Lamb shift in muonic hydrogen,''
  Phys.\ Rev.\ A {\bf 84}, 020102 (2011)
  [arXiv:1101.5965 [hep-ph]].
  %%CITATION = ARXIV:1101.5965;%%
   
%\cite{Alarcon:2013cba}
\bibitem{Alarcon:2013cba} 
  J.~M.~Alarc\'on, V.~Lensky and V.~Pascalutsa,
  %``Chiral perturbation theory of muonic hydrogen Lamb shift: polarizability contribution,''
  arXiv:1312.1219 [hep-ph].
  %%CITATION = ARXIV:1312.1219;%%
 
%\cite{Bernard:2002pw}
\bibitem{Bernard:2002pw} 
  V.~Bernard, T.~R.~Hemmert and U.~G.~Meissner,
  %``Spin structure of the nucleon at low-energies,''
  Phys.\ Rev.\ D {\bf 67}, 076008 (2003)
  [hep-ph/0212033].
  %%CITATION = HEP-PH/0212033;%%
 
%\cite{Birse:2012eb}
\bibitem{Birse:2012eb} 
  M.~C.~Birse and J.~A.~McGovern,
  %``Proton polarisability contribution to the Lamb shift in muonic hydrogen at fourth order in chiral perturbation theory,''
  Eur.\ Phys.\ J.\ A {\bf 48}, 120 (2012)
  [arXiv:1206.3030 [hep-ph]].
  %%CITATION = ARXIV:1206.3030;%%
 
%\cite{Hill:2011wy}
\bibitem{Hill:2011wy} 
  R.~J.~Hill and G.~Paz,
  %``Model independent analysis of proton structure for hydrogenic bound states,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 160402 (2011)
  [arXiv:1103.4617 [hep-ph]].
  %%CITATION = ARXIV:1103.4617;%% 

  %\cite{Hemmert:1996xg}
\bibitem{Hemmert:1996xg}
  T.~R.~Hemmert, B.~R.~Holstein and J.~Kambor,
  %``Systematic 1/M expansion for spin 3/2 particles in baryon chiral perturbation theory,''
  Phys.\ Lett.\ B {\bf 395} (1997) 89
  [hep-ph/9606456].
  %%CITATION = HEP-PH/9606456;%%
  
  %\cite{Hemmert:1997ye}
\bibitem{Hemmert:1997ye}
  T.~R.~Hemmert, B.~R.~Holstein and J.~Kambor,
  %``Chiral Lagrangians and delta(1232) interactions: Formalism,''
  J.\ Phys.\ G {\bf 24} (1998) 1831
  [hep-ph/9712496].
  %%CITATION = HEP-PH/9712496;%%
  
%\cite{Ji:1999mr}
\bibitem{Ji:1999mr}
  X.~-D.~Ji and J.~Osborne,
  %``Generalized sum rules for spin dependent structure functions of the nucleon,''
  J.\ Phys.\ G {\bf 27} (2001) 127
  [hep-ph/9905410].
  %%CITATION = HEP-PH/9905410;%%
 



  
 
%\cite{Peset:2014yha}
\bibitem{Peset:2014yha} 
  C.~Peset and A.~Pineda,
  %``Model independent determination of the muonic hydrogen Lamb shift and proton radius,''
  arXiv:1403.3408 [hep-ph].
  %%CITATION = ARXIV:1403.3408;%%

\bibitem{Weise} T. Ericson and W. Weise, {\it Pions and Nuclei},
Ed. Oxford Univ. Press (1988).
  
  %\cite{Bernard:1995dp}
\bibitem{Bernard:1995dp}
  V.~Bernard, N.~Kaiser and U.~-G.~Meissner,
  %``Chiral dynamics in nucleons and nuclei,''
  Int.\ J.\ Mod.\ Phys.\ E {\bf 4} (1995) 193
  [hep-ph/9501384].
  %%CITATION = HEP-PH/9501384;%%

  %\cite{Hemmert:1996rw}
\bibitem{Hemmert:1996rw}
  T.~R.~Hemmert, B.~R.~Holstein and J.~Kambor,
  %``Delta (1232) and the polarizabilities of the nucleon,''
  Phys.\ Rev.\ D {\bf 55} (1997) 5598
  [hep-ph/9612374].
  %%CITATION = HEP-PH/9612374;%%

\bibitem{BKKM} H.W. Fearing, R. Lewis, N. Mobed
and S. Scherer, Phys. Rev. {\bf D56}, 1783 (1997).

\bibitem{BFHM} V. Bernard, H.W. Fearing, T.R. Hemmert and U.-G.
Meissner, Nucl. Phys. {\bf A635}, 121 (1998); E-{\it ibid.}, {\bf
A642}, 563 (1998).  
 
%\cite{Scherer:1996ux}
\bibitem{Scherer:1996ux} 
  S.~Scherer, A.~Y.~.Korchin and J.~H.~Koch,
  %``Virtual Compton scattering off the nucleon at low-energies,''
  Phys.\ Rev.\ C {\bf 54}, 904 (1996)
  [nucl-th/9605030].
  %%CITATION = NUCL-TH/9605030;%%

%\cite{Fearing:1996gs}
\bibitem{Fearing:1996gs} 
  H.~W.~Fearing and S.~Scherer,
  %``Virtual Compton scattering off spin zero particles at low-energies,''
  Few Body Syst.\  {\bf 23}, 111 (1998)
  [nucl-th/9607056].
  %%CITATION = NUCL-TH/9607056;%%

 

%\cite{Bernabeu:1973uf}
\bibitem{Bernabeu:1973uf} 
  J.~Bernabeu and C.~Jarlskog,
  %``Polarizability Contribution To The Energy Levels Of The Muonic Helium (mu He-4)+,''
  Nucl.\ Phys.\ B {\bf 75}, 59 (1974).
  %%CITATION = NUPHA,B75,59;%%

%\cite{Janssens:1965kd}
\bibitem{Janssens:1965kd} 
  T.~Janssens, R.~Hofstadter, E.~B.~Hughes and M.~R.~Yearian,
  %``Proton form factors from elastic electron-proton scattering,''
  Phys.\ Rev.\  {\bf 142}, 922 (1966).
  %%CITATION = PHRVA,142,922;%%

%\cite{Kelly:2004hm}
\bibitem{Kelly:2004hm} 
  J.~J.~Kelly,
  %``Simple parametrization of nucleon form factors,''
  Phys.\ Rev.\ C {\bf 70}, 068202 (2004).
  %%CITATION = PHRVA,C70,068202;%%

%\cite{Distler:2010zq}
\bibitem{Distler:2010zq} 
  M.~O.~Distler, J.~C.~Bernauer and T.~Walcher,
  %``The RMS Charge Radius of the Proton and Zemach Moments,''
  Phys.\ Lett.\ B {\bf 696}, 343 (2011)
  [arXiv:1011.1861 [nucl-th]].
  %%CITATION = ARXIV:1011.1861;%%

%\cite{Friar:2005jz}
\bibitem{Friar:2005jz} 
  J.~L.~Friar and I.~Sick,
  %``Muonic hydrogen and the third Zemach moment,''
  Phys.\ Rev.\ A {\bf 72}, 040502 (2005)
  [nucl-th/0508025].
  %%CITATION = NUCL-TH/0508025;%%

%\cite{Bernauer:2010wm}
\bibitem{Bernauer:2010wm} 
  J.~C.~Bernauer {\it et al.}  [A1 Collaboration],
  %``High-precision determination of the electric and magnetic form factors of the proton,''
  Phys.\ Rev.\ Lett.\  {\bf 105}, 242001 (2010)
  [arXiv:1007.5076 [nucl-ex]].
  %%CITATION = ARXIV:1007.5076;%%

%\cite{Lorenz:2012tm}
\bibitem{Lorenz:2012tm} 
  I.~T.~Lorenz, H.~-W.~Hammer and U.~-G.~Meissner,
  %``The size of the proton - closing in on the radius puzzle,''
  Eur.\ Phys.\ J.\ A {\bf 48}, 151 (2012)
  [arXiv:1205.6628 [hep-ph]].
  %%CITATION = ARXIV:1205.6628;%%

%\cite{Martynenko:2005rc}
\bibitem{Martynenko:2005rc} 
  A.~P.~Martynenko,
  %``Proton polarizability effect in the Lamb shift of the hydrogen atom,''
  Phys.\ Atom.\ Nucl.\  {\bf 69}, 1309 (2006)
  [hep-ph/0509236].
  %%CITATION = HEP-PH/0509236;%%


%\cite{Gorchtein:2013yga}
\bibitem{Gorchtein:2013yga} 
  M.~Gorchtein, F.~J.~Llanes-Estrada and A.~P.~Szczepaniak,
  %``$\mu-H$ Lamb shift: dispersing the nucleon-excitation uncertainty with a finite energy sum rule,''
  Phys.\ Rev.\ A {\bf 87}, 052501 (2013)
  [arXiv:1302.2807 [nucl-th]].
  %%CITATION = ARXIV:1302.2807;%%

%\cite{Friar:1997tr}
\bibitem{Friar:1997tr}
J.~L.~Friar and G.~L.~Payne,
%``Higher-Order Nuclear-Polarizability Corrections in Atomic Hydrogen,''
Phys.\ Rev.\ C {\bf 56}, 619 (1997)
[arXiv:nucl-th/9704032].
%%CITATION = NUCL-TH 9704032;%%

\bibitem{KS} I.B. Khriplovich and R.A. Sen'kov, Phys. Lett. {\bf A249}, 474 (1998). 

%\cite{Hemmert:1999pz}
\bibitem{Hemmert:1999pz}
T.~R.~Hemmert, B.~R.~Holstein, G.~Knochlein and D.~Drechsel,
%``Generalized polarizabilities of the nucleon in chiral effective  theories,''
Phys.\ Rev.\ D {\bf 62}, 014013 (2000)
[arXiv:nucl-th/9910036].
%%CITATION = NUCL-TH 9910036;%%

%\cite{Beringer:1900zz}
\bibitem{Beringer:1900zz} 
  J.~Beringer {\it et al.}  [Particle Data Group Collaboration],
  %``Review of Particle Physics (RPP),''
  Phys.\ Rev.\ D {\bf 86}, 010001 (2012).
  %%CITATION = PHRVA,D86,010001;%%



\bibitem{DS} S.D. Drell and J.D. Sullivan, Phys. Rev. {\bf 154}, 1477 (1967).
  

\bibitem{Zemach} A.C. Zemach, Phys. Rev. {\bf 104}, 1771 (1956).

%\cite{DeRafael:1971mc}
\bibitem{DeRafael:1971mc} 
  E.~De Rafael,
  %``The hydrogen hyperfine structure and inelastic electron proton scattering experiments,''
  Phys.\ Lett.\ B {\bf 37}, 201 (1971).
  %%CITATION = PHLTA,B37,201;%%

%\cite{Faustov:2001pn}
\bibitem{Faustov:2001pn} 
  R.~N.~Faustov, E.~V.~Cherednikova and A.~P.~Martynenko,
  %``Proton polarizability contribution to the hyperfine splitting in muonic hydrogen,''
  Nucl.\ Phys.\ A {\bf 703}, 365 (2002)
  [hep-ph/0108044].
  %%CITATION = HEP-PH/0108044;%%

%\cite{Carlson:2008ke}
\bibitem{Carlson:2008ke} 
  C.~E.~Carlson, V.~Nazaryan and K.~Griffioen,
  %``Proton structure corrections to electronic and muonic hydrogen hyperfine splitting,''
  Phys.\ Rev.\ A {\bf 78}, 022517 (2008)
  [arXiv:0805.2603 [physics.atom-ph]].
  %%CITATION = ARXIV:0805.2603;%%

\bibitem{KarlPaton} G. Karl and J.E. Paton, Phys. Rev. {\bf D30}, 238
(1984).  

%\cite{Dupays:2003zz}
\bibitem{Dupays:2003zz} 
  A.~Dupays, A.~Beswick, B.~Lepetit, C.~Rizzo and D.~Bakalov,
  %``Proton Zemach radius from measurements of the hyperfine splitting of hydrogen and muonic hydrogen,''
  Phys.\ Rev.\ A {\bf 68}, 052503 (2003).
  %%CITATION = PHRVA,A68,052503;%%
    
%\cite{Volotka:2004zu}
\bibitem{Volotka:2004zu} 
  A.~V.~Volotka, V.~M.~Shabaev, G.~Plunien and G.~Soff,
  %``Zemach and magnetic radius of the proton from the hyperfine splitting in hydrogen,''
  Eur.\ Phys.\ J.\ D {\bf 33}, 23 (2005)
  [physics/0405118].
  %%CITATION = PHYSICS/0405118;%%
 


%\cite{Lorenz:2014yda}
\bibitem{Lorenz:2014yda} 
  I.~T.~Lorenz, U.~G.~Mei{\ss}ner, H.-W.~Hammer and Y.-B.~Dong,
  %``Theoretical Constraints and Systematic Effects in the Determination of the Proton Form Factors,''
  Phys.\ Rev.\ D {\bf 91}, no. 1, 014023 (2015)
  [arXiv:1411.1704 [hep-ph]].
  %%CITATION = ARXIV:1411.1704;%%






%\cite{Manohar:1997qy}
\bibitem{Manohar:1997qy} 
  A.~V.~Manohar,
  %``The HQET / NRQCD Lagrangian to order alpha / m-3,''
  Phys.\ Rev.\ D {\bf 56}, 230 (1997)
  [hep-ph/9701294].
  %%CITATION = HEP-PH/9701294;%%

 

%\cite{Agashe:2014kda}
\bibitem{Agashe:2014kda}
  K.~A.~Olive {\it et al.} [Particle Data Group Collaboration],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 38} (2014) 090001.
  %%CITATION = CHPHD,C38,090001;%%
 
 
%\cite{Pineda:1998kj}
\bibitem{Pineda:1998kj}
  A.~Pineda and J.~Soto,
  %``Matching at one loop for the four quark operators in NRQCD,''
  Phys.\ Rev.\ D {\bf 58} (1998) 114011
  [hep-ph/9802365].
  %%CITATION = HEP-PH/9802365;%%
   



%\cite{Kallen:1955fb}
\bibitem{Kallen:1955fb} 
  A.~O G.~Kallen and A.~Sabry,
  %``Fourth order vacuum polarization,''
  Kong.\ Dan.\ Vid.\ Sel.\ Mat.\ Fys.\ Med.\  {\bf 29N17}, 1 (1955).
  %%CITATION = KDVSA,29N17,1;%%

%\cite{Kinoshita:1979dy}
\bibitem{Kinoshita:1979dy}
T.~Kinoshita and W.~B.~Lindquist,
%``Parametric Formula For The Sixth Order Vacuum Polarization Contribution In
%Quantum Electrodynamics,''
Phys.\ Rev.\ D {\bf 27}, 853 (1983).
%%CITATION = PHRVA,D27,853;%%




 %\cite{Pineda:2011dg}
\bibitem{Pineda:2011dg} 
  A.~Pineda,
  %``Review of Heavy Quarkonium at weak coupling,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 67}, 735 (2012)
  [arXiv:1111.0165 [hep-ph]].
  %%CITATION = ARXIV:1111.0165;%%

  
 
  \bibitem{Pachucki96} K. Pachucki, Phys. Rev. {\bf A53}, 2092 (1996).
    
%\cite{Hoang:2000fm}
\bibitem{Hoang:2000fm} 
  A.~H.~Hoang,
  %``Bottom quark mass from Upsilon mesons: Charm mass effects,''
  hep-ph/0008102.
  %%CITATION = HEP-PH/0008102;%%




\bibitem{KMY}
I.~B.~Khriplovich, A.~I.~Milstein and A.~S.~Yelkhovsky, Phys. Scr. Vol T46 (1993) 252.
 

%\cite{Antognini:2013jkc}
\bibitem{Antognini:2013jkc} 
  A.~Antognini, F.~Kottmann, F.~Biraben, P.~Indelicato, F.~Nez and R.~Pohl,
  %``Theory of the 2S-2P Lamb shift and 2S hyperfine splitting in muonic hydrogen,''
  Annals Phys.\  {\bf 331}, 127 (2013)
  [arXiv:1208.2637 [physics.atom-ph]].
  %%CITATION = ARXIV:1208.2637;%%

\bibitem{GRS} 
S.~N. Gupta, W.~W. Repko, and C.J. Suchyta, III,
Phys. Rev. D {\bf 40}, 4100 (1989).  

%\cite{Pineda:1997bj}
\bibitem{Pineda:1997bj} 
  A.~Pineda and J.~Soto,
  %``Effective field theory for ultrasoft momenta in NRQCD and NRQED,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 64}, 428 (1998)
  [hep-ph/9707481].
  %%CITATION = HEP-PH/9707481;%%

%\cite{Brambilla:1999xf}
\bibitem{Brambilla:1999xf} 
  N.~Brambilla, A.~Pineda, J.~Soto and A.~Vairo,
  %``Potential NRQCD: An Effective theory for heavy quarkonium,''
  Nucl.\ Phys.\ B {\bf 566}, 275 (2000)
  [hep-ph/9907240].
  %%CITATION = HEP-PH/9907240;%%

%\cite{Brambilla:2004jw}
\bibitem{Brambilla:2004jw} 
  N.~Brambilla, A.~Pineda, J.~Soto and A.~Vairo,
  %``Effective field theories for heavy quarkonium,''
  Rev.\ Mod.\ Phys.\  {\bf 77}, 1423 (2005)
  [hep-ph/0410047].
  %%CITATION = HEP-PH/0410047;%%

%\cite{Pineda:2011dg}
\bibitem{Pineda:2011dg}
  A.~Pineda,
  %``Review of Heavy Quarkonium at weak coupling,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 67} (2012) 735
  [arXiv:1111.0165 [hep-ph]].
  %%CITATION = ARXIV:1111.0165;%%

%\cite{Caswell:1985ui}
\bibitem{Caswell:1985ui} 
  W.~E.~Caswell and G.~P.~Lepage,
  %``Effective Lagrangians for Bound State Problems in QED, QCD, and Other Field Theories,''
  Phys.\ Lett.\ B {\bf 167}, 437 (1986).
  %%CITATION = PHLTA,B167,437;%%

%\cite{Bodwin:1994jh}
\bibitem{Bodwin:1994jh} 
  G.~T.~Bodwin, E.~Braaten and G.~P.~Lepage,
  %``Rigorous QCD analysis of inclusive annihilation and production of heavy quarkonium,''
  Phys.\ Rev.\ D {\bf 51}, 1125 (1995)
  [Phys.\ Rev.\ D {\bf 55}, 5853 (1997)]
  [hep-ph/9407339].
  %%CITATION = HEP-PH/9407339;%%

%\cite{Brambilla:2000gk}
\bibitem{Brambilla:2000gk}
  N.~Brambilla, A.~Pineda, J.~Soto and A.~Vairo,
  %``The QCD potential at O(1/m),''
  Phys.\ Rev.\ D {\bf 63} (2001) 014023
  [hep-ph/0002250].
  %%CITATION = HEP-PH/0002250;%%
  
  %\cite{Pineda:2000sz}
\bibitem{Pineda:2000sz}
  A.~Pineda and A.~Vairo,
  %``The QCD potential at O (1 / $m^{2)}$ : Complete spin dependent and spin independent result,''
  Phys.\ Rev.\ D {\bf 63} (2001) 054007
   [Phys.\ Rev.\ D {\bf 64} (2001) 039902]
  [hep-ph/0009145].
  %%CITATION = HEP-PH/0009145;%%

%\cite{Wilson:1974sk}
\bibitem{Wilson:1974sk} 
  K.~G.~Wilson,
  %``Confinement of Quarks,''
  Phys.\ Rev.\ D {\bf 10}, 2445 (1974).
  %%CITATION = PHRVA,D10,2445;%%

%\cite{Kniehl:2002br}
\bibitem{Kniehl:2002br} 
  B.~A.~Kniehl, A.~A.~Penin, V.~A.~Smirnov and M.~Steinhauser,
  %``Potential NRQCD and heavy quarkonium spectrum at next-to-next-to-next-to-leading order,''
  Nucl.\ Phys.\ B {\bf 635}, 357 (2002)
  [hep-ph/0203166].
  %%CITATION = HEP-PH/0203166;%%

%\cite{Gupta:1981pd}
\bibitem{Gupta:1981pd} 
  S.~N.~Gupta and S.~F.~Radford,
  %``Quark Quark and Quark - Anti-quark Potentials,''
  Phys.\ Rev.\ D {\bf 24}, 2309 (1981).
  %%CITATION = PHRVA,D24,2309;%%

\bibitem{Pantaleone:1985uf}
  J.~T.~Pantaleone, S.~H.~H.~Tye and Y.~J.~Ng,
  %``Spin Splittings in Heavy Quarkonia,''
  Phys.\ Rev.\ D {\bf 33} (1986) 777.
  %%CITATION = PHRVA,D33,777;%%

%\cite{Titard:1993nn}
\bibitem{Titard:1993nn} 
  S.~Titard and F.~J.~Yndurain,
  %``Rigorous QCD evaluation of spectrum and ground state properties of heavy q anti-q systems: With a precision determination of m(b) M(eta(b)),''
  Phys.\ Rev.\ D {\bf 49}, 6007 (1994)
  [hep-ph/9310236].
  %%CITATION = HEP-PH/9310236;%%

%\cite{Manohar:2000hj}
\bibitem{Manohar:2000hj} 
  A.~V.~Manohar and I.~W.~Stewart,
  %``The QCD heavy quark potential to order v**2: One loop matching conditions,''
  Phys.\ Rev.\ D {\bf 62}, 074015 (2000)
  [hep-ph/0003032].
  %%CITATION = HEP-PH/0003032;%%

  %\cite{Kniehl:2001ju}
\bibitem{Kniehl:2001ju}
  B.~A.~Kniehl, A.~A.~Penin, M.~Steinhauser and V.~A.~Smirnov,
  %``NonAbelian alpha**3(s) / (m(q)r**2) heavy quark anti-quark potential,''
  Phys.\ Rev.\ D {\bf 65} (2002) 091503
  [hep-ph/0106135].
  %%CITATION = HEP-PH/0106135;%%
  
 %\cite{Beneke:1997zp}
\bibitem{Beneke:1997zp} 
  M.~Beneke and V.~A.~Smirnov,
  %``Asymptotic expansion of Feynman integrals near threshold,''
  Nucl.\ Phys.\ B {\bf 522}, 321 (1998)
  [hep-ph/9711391].
  %%CITATION = HEP-PH/9711391;%%

%\cite{Pineda:1997ie}
\bibitem{Pineda:1997ie} 
  A.~Pineda and J.~Soto,
  %``The Lamb shift in dimensional regularization,''
  Phys.\ Lett.\ B {\bf 420}, 391 (1998)
  [hep-ph/9711292].
  %%CITATION = HEP-PH/9711292;%%

%\cite{Pineda:1998kn}
\bibitem{Pineda:1998kn} 
  A.~Pineda and J.~Soto,
  %``Potential NRQED: The Positronium case,''
  Phys.\ Rev.\ D {\bf 59}, 016005 (1999)
  [hep-ph/9805424].
  %%CITATION = HEP-PH/9805424;%%

%\cite{Brambilla:1999xj}
\bibitem{Brambilla:1999xj} 
  N.~Brambilla, A.~Pineda, J.~Soto and A.~Vairo,
  %``The Heavy quarkonium spectrum at order m alpha**5(s) l n alpha(s),''
  Phys.\ Lett.\ B {\bf 470}, 215 (1999)
  [hep-ph/9910238].
  %%CITATION = HEP-PH/9910238;%%

%\cite{Fischler:1977yf}
\bibitem{Fischler:1977yf} 
  W.~Fischler,
  %``Quark - anti-Quark Potential in QCD,''
  Nucl.\ Phys.\ B {\bf 129}, 157 (1977).
  %%CITATION = NUPHA,B129,157;%%
        
%\cite{Schroder:1998vy}
\bibitem{Schroder:1998vy}
  Y.~Schroder,
  %``The Static potential in QCD to two loops,''
  Phys.\ Lett.\ B {\bf 447} (1999) 321
  [hep-ph/9812205].
  %%CITATION = HEP-PH/9812205;%%

%\cite{Brambilla:1999qa}
\bibitem{Brambilla:1999qa} 
  N.~Brambilla, A.~Pineda, J.~Soto and A.~Vairo,
  %``The Infrared behavior of the static potential in perturbative QCD,''
  Phys.\ Rev.\ D {\bf 60}, 091502 (1999)
  [hep-ph/9903355].
  %%CITATION = HEP-PH/9903355;%%

%\cite{Anzai:2009tm}
\bibitem{Anzai:2009tm}
  C.~Anzai, Y.~Kiyo, Y.~Sumino,
  %``Static QCD potential at three-loop order,''
  Phys.\ Rev.\ Lett.\  {\bf 104}, 112003 (2010).
  [arXiv:0911.4335 [hep-ph]].

%\cite{Smirnov:2009fh}
\bibitem{Smirnov:2009fh}
  A.~V.~Smirnov, V.~A.~Smirnov, M.~Steinhauser,
  %``Three-loop static potential,''
  Phys.\ Rev.\ Lett.\  {\bf 104}, 112002 (2010).
  [arXiv:0911.4742 [hep-ph]].

%\cite{Manohar:1997qy}
\bibitem{Manohar:1997qy} 
  A.~V.~Manohar,
  %``The HQET / NRQCD Lagrangian to order alpha / m-3,''
  Phys.\ Rev.\ D {\bf 56}, 230 (1997)
  [hep-ph/9701294].
  %%CITATION = HEP-PH/9701294;%%

%\cite{Bauer:1997gs}
\bibitem{Bauer:1997gs} 
  C.~W.~Bauer and A.~V.~Manohar,
  %``Renormalization group scaling of the 1/m**2 HQET Lagrangian,''
  Phys.\ Rev.\ D {\bf 57}, 337 (1998)
  [hep-ph/9708306].
  %%CITATION = HEP-PH/9708306;%%

%\cite{Beneke:2013jia}
\bibitem{Beneke:2013jia} 
  M.~Beneke, Y.~Kiyo and K.~Schuller,
  %``Third-order correction to top-quark pair production near threshold I. Effective theory set-up and matching coefficients,''
  arXiv:1312.4791 [hep-ph].
  %%CITATION = ARXIV:1312.4791;%%

%\cite{Eichten:1990vp}
\bibitem{Eichten:1990vp} 
  E.~Eichten and B.~R.~Hill,
  %``STATIC EFFECTIVE FIELD THEORY: 1/m CORRECTIONS,''
  Phys.\ Lett.\ B {\bf 243}, 427 (1990).
  %%CITATION = PHLTA,B243,427;%%

%\cite{Pineda:1998kj}
\bibitem{Pineda:1998kj}
  A.~Pineda and J.~Soto,
  %``Matching at one loop for the four quark operators in NRQCD,''
  Phys.\ Rev.\ D {\bf 58} (1998) 114011
  [hep-ph/9802365].
  %%CITATION = HEP-PH/9802365;%%

%\cite{Pineda:2001ra}
\bibitem{Pineda:2001ra} 
  A.~Pineda,
  %``Renormalization group improvement of the NRQCD Lagrangian and heavy quarkonium spectrum,''
  Phys.\ Rev.\ D {\bf 65}, 074007 (2002)
  [hep-ph/0109117].
  %%CITATION = HEP-PH/0109117;%%
  
%\cite{Schroder:1999sg}
\bibitem{Schroder:1999sg} 
  Y.~Schroder,
  %``The Static potential in QCD,''
  DESY-THESIS-1999-021.
  %%CITATION = DESY-THESIS-1999-021;%%  
  
  %\cite{ThesisPeset}
\bibitem{ThesisPeset} 
  C.~Peset,
  %``The Static potential in QCD,''
  PhD thesis, {\it in preparation}.
    
  %\cite{Luke:1999kz}
\bibitem{Luke:1999kz} 
  M.~E.~Luke, A.~V.~Manohar and I.~Z.~Rothstein,
  %``Renormalization group scaling in nonrelativistic QCD,''
  Phys.\ Rev.\ D {\bf 61}, 074025 (2000)
  [hep-ph/9910209].
  %%CITATION = HEP-PH/9910209;%%
  
%\cite{Eichten:1980mw}
\bibitem{Eichten:1980mw} 
  E.~Eichten and F.~Feinberg,
  %``Spin Dependent Forces in QCD,''
  Phys.\ Rev.\ D {\bf 23}, 2724 (1981).
  %%CITATION = PHRVA,D23,2724;%%
 
%\cite{Barchielli:1986zs}
\bibitem{Barchielli:1986zs} 
  A.~Barchielli, E.~Montaldi and G.~M.~Prosperi,
  %``On a Systematic Derivation of the Quark - Anti-quark Potential,''
  Nucl.\ Phys.\ B {\bf 296}, 625 (1988)
  [Nucl.\ Phys.\ B {\bf 303}, 752 (1988)].
  %%CITATION = NUPHA,B296,625;%%

%\cite{Barchielli:1988zp}
\bibitem{Barchielli:1988zp} 
  A.~Barchielli, N.~Brambilla and G.~M.~Prosperi,
  %``Relativistic Corrections to the Quark - anti-Quark Potential and the Quarkonium Spectrum,''
  Nuovo Cim.\ A {\bf 103}, 59 (1990).
  %%CITATION = NUCIA,A103,59;%%

%\cite{Chen:1994dg}
\bibitem{Chen:1994dg} 
  Y.~Q.~Chen, Y.~P.~Kuang and R.~J.~Oakes,
  %``On the spin dependent potential between heavy quark and anti-quark,''
  Phys.\ Rev.\ D {\bf 52}, 264 (1995)
  [hep-ph/9406287].
  %%CITATION = HEP-PH/9406287;%%

%\cite{Beneke:1999qg}
\bibitem{Beneke:1999qg} 
  M.~Beneke, A.~Signer and V.~A.~Smirnov,
  %``Top quark production near threshold and the top quark mass,''
  Phys.\ Lett.\ B {\bf 454}, 137 (1999)
  [hep-ph/9903260].
  %%CITATION = HEP-PH/9903260;%%

%\cite{Beneke:2014qea}
\bibitem{Beneke:2014qea} 
  M.~Beneke, Y.~Kiyo, P.~Marquard, A.~Penin, J.~Piclum, D.~Seidel and M.~Steinhauser,
  %``Leptonic decay of the $\Upsilon$(1$S$) meson at third order in QCD,''
  Phys.\ Rev.\ Lett.\  {\bf 112}, no. 15, 151801 (2014)
  [arXiv:1401.3005 [hep-ph]].
  %%CITATION = ARXIV:1401.3005;%%

%\cite{Kniehl:1999ud}
\bibitem{Kniehl:1999ud} 
  B.~A.~Kniehl and A.~A.~Penin,
  %``Ultrasoft effects in heavy quarkonium physics,''
  Nucl.\ Phys.\ B {\bf 563}, 200 (1999)
  [hep-ph/9907489].
  %%CITATION = HEP-PH/9907489;%%

%\cite{Brambilla:2002nu}
\bibitem{Brambilla:2002nu} 
  N.~Brambilla, D.~Eiras, A.~Pineda, J.~Soto and A.~Vairo,
  %``Inclusive decays of heavy quarkonium to light particles,''
  Phys.\ Rev.\ D {\bf 67}, 034018 (2003)
  [hep-ph/0208019].
  %%CITATION = HEP-PH/0208019;%%

%\cite{Pineda:2000gza}
\bibitem{Pineda:2000gza} 
  A.~Pineda and J.~Soto,
  %``The Renormalization group improvement of the QCD static potentials,''
  Phys.\ Lett.\ B {\bf 495}, 323 (2000)
  %doi:10.1016/S0370-2693(00)01261-2
  [hep-ph/0007197].
  %%CITATION = doi:10.1016/S0370-2693(00)01261-2;%%

%\cite{Brambilla:2001xk}
\bibitem{Brambilla:2001xk}
  N.~Brambilla, D.~Gromes and A.~Vairo,
  %``Poincare invariance and the heavy quark potential,''
  Phys.\ Rev.\ D {\bf 64} (2001) 076010
  [hep-ph/0104068].
  %%CITATION = HEP-PH/0104068;%%

%\cite{Brambilla:2003nt}
\bibitem{Brambilla:2003nt} 
  N.~Brambilla, D.~Gromes and A.~Vairo,
  %``Poincare invariance constraints on NRQCD and potential NRQCD,''
  Phys.\ Lett.\ B {\bf 576}, 314 (2003)
  [hep-ph/0306107].
  %%CITATION = HEP-PH/0306107;%%

%\cite{Buchmuller:1981aj}
\bibitem{Buchmuller:1981aj}
  W.~Buchmuller, Y.~J.~Ng and S.~H.~H.~Tye,
  %``Hyperfine Splittings in Heavy Quark Systems,''
  Phys.\ Rev.\ D {\bf 24} (1981) 3003.
  %%CITATION = PHRVA,D24,3003;%%
 
%\cite{Kiyo:2014uca}
\bibitem{Kiyo:2014uca}
  Y.~Kiyo and Y.~Sumino,
  %``Full Formula for Heavy Quarkonium Energy Levels at Next-to-next-to-next-to-leading Order,''
  Nucl.\ Phys.\ B {\bf 889} (2014) 156
  [arXiv:1408.5590 [hep-ph]].
  %%CITATION = ARXIV:1408.5590;%%

\bibitem{Penin:2002zv}
  A.~A.~Penin and M.~Steinhauser,
  %``Heavy quarkonium spectrum at O(alpha**5(s) m(q)) and bottom / top quark mass determination,''
  Phys.\ Lett.\ B {\bf 538} (2002) 335
  [hep-ph/0204290].
  %%CITATION = HEP-PH/0204290;%%
 
%\cite{Penin:2005eu}
\bibitem{Penin:2005eu} 
  A.~A.~Penin, V.~A.~Smirnov and M.~Steinhauser,
  %``Heavy quarkonium spectrum and production/annihilation rates to order beta**3(0) alpha**3(s),''
  Nucl.\ Phys.\ B {\bf 716}, 303 (2005)
  [hep-ph/0501042].
  %%CITATION = HEP-PH/0501042;%%

%\cite{Beneke:2005hg}
\bibitem{Beneke:2005hg} 
  M.~Beneke, Y.~Kiyo and K.~Schuller,
  %``Third-order Coulomb corrections to the S-wave Green function, energy levels and wave functions at the origin,''
  Nucl.\ Phys.\ B {\bf 714}, 67 (2005)
  [hep-ph/0501289].
  %%CITATION = HEP-PH/0501289;%%

%\cite{Brambilla:2000db}
\bibitem{Brambilla:2000db}
  N.~Brambilla and A.~Vairo,
  %``The $B_c$ mass up to order $\alpha($s$)^{4}$,''
  Phys.\ Rev.\ D {\bf 62} (2000) 094019
  [hep-ph/0002075].
  %%CITATION = HEP-PH/0002075;%%

%\cite{Brambilla:2001qk}
\bibitem{Brambilla:2001qk} 
  N.~Brambilla, Y.~Sumino and A.~Vairo,
  %``Quarkonium spectroscopy and perturbative QCD: Massive quark loop effects,''
  Phys.\ Rev.\ D {\bf 65}, 034001 (2002)
  [hep-ph/0108084].
  %%CITATION = HEP-PH/0108084;%%

%\cite{Pineda:1997hz}
\bibitem{Pineda:1997hz} 
  A.~Pineda and F.~J.~Yndurain,
  %``Calculation of quarkonium spectrum and m(b), m(c) to order alpha-s**4,''
  Phys.\ Rev.\ D {\bf 58}, 094022 (1998)
  [hep-ph/9711287].
  %%CITATION = HEP-PH/9711287;%%

   %\cite{Kiyo:2013aea}
\bibitem{Kiyo:2013aea}
  Y.~Kiyo and Y.~Sumino,
  %``Perturbative heavy quarkonium spectrum at next-to-next-to-next-to-leading order,''
  Phys.\ Lett.\ B {\bf 730} (2014) 76
  [arXiv:1309.6571 [hep-ph]].
  %%CITATION = ARXIV:1309.6571;%%

%\cite{Bali:1997am}
\bibitem{Bali:1997am} 
  G.~S.~Bali, K.~Schilling and A.~Wachter,
  %``Complete O (v**2) corrections to the static interquark potential from SU(3) gauge theory,''
  Phys.\ Rev.\ D {\bf 56}, 2566 (1997)
  [hep-lat/9703019].
  %%CITATION = HEP-LAT/9703019;%%

%\cite{Koma:2007jq}
\bibitem{Koma:2007jq} 
  Y.~Koma, M.~Koma and H.~Wittig,
  %``Relativistic corrections to the static potential at O(1/m) and O(1/m**2),''
  PoS LAT {\bf 2007}, 111 (2007)
  [arXiv:0711.2322 [hep-lat]].
  %%CITATION = ARXIV:0711.2322;%%

%\cite{Koma:2009ws}
\bibitem{Koma:2009ws} 
  Y.~Koma and M.~Koma,
  %``Scaling study of the relativistic corrections to the static potential,''
  PoS LAT {\bf 2009}, 122 (2009)
  [arXiv:0911.3204 [hep-lat]].
  %%CITATION = ARXIV:0911.3204;%%
    
  %\cite{Manohar:2000kr}
\bibitem{Manohar:2000kr} 
  A.~V.~Manohar and I.~W.~Stewart,
  %``Running of the heavy quark production current and 1 / v potential in QCD,''
  Phys.\ Rev.\ D {\bf 63}, 054004 (2001)
  [hep-ph/0003107].
  %%CITATION = HEP-PH/0003107;%%
 
 
\end{thebibliography}





==> Introduction/introduction.tex <==
\chapter*{Introduction}


In summary, this thesis is divided into two main parts.



==> Title/title.tex <==
\begin{titlepage}
\begin{center}

% logos %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\includegraphics[height=10mm]{Title/IFAE_logo.eps}
\hfill
\includegraphics[height=10mm]{Title/uab_logo.eps}
\end{figure}

% title %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{0.5cm}
\HRule\\
\vspace{0.2cm}
{\huge \bf Effective field theories for heavy quarkonia and hydrogen-like bound states}
\HRule\\
\par
\vspace{1.5in}

% author %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\LARGE \bf Clara Peset Mart\'in}
\vspace{0.3cm}
\par
{\large \bf Ph.D. thesis}\\
Institut de F\'{i}sica d'Altes Energies\\
Universitat Aut\`{o}noma de Barcelona\\
Departament de F\'{i}sica\\
Facultat de Ci\`{e}ncies \\
%Edifici Cn E-08193 Bellaterra (Barcelona)
\par
\vspace{0.5in}

% date %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\today
%December 20, 2011
%\date 
\par
\vspace{0.5in}

% supervisor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \vfill
\emph{Supervisor:}\\
{\bf Prof. Antonio Pineda Ru\'iz}\\
Grup de F\'{i}sica Te\`{o}rica\\
Departament de F\'{i}sica\\
Universitat Aut\`{o}noma de Barcelona\\



\end{center}
\end{titlepage}



==> papers/papers.tex <==
.........\\
........\\

.....

